mmPred: Radar-based Human Motion Prediction in the Dark

Existing Human Motion Prediction (HMP) methods based on RGB-D cameras are sensitive to lighting conditions and raise privacy concerns, limiting their real-world applications such as firefighting and healthcare. Motivated by the robustness and privacy-preserving nature of millimeter-wave (mmWave) radar, this work introduces radar as a novel sensing modality for HMP, for the first time. Nevertheless, radar signals often suffer from specular reflections and multipath effects, resulting in noisy and temporally inconsistent measurements, such as body-part miss-detection. To address these radar-specific artifacts, we propose mmPred, the first diffusion-based framework tailored for radar-based HMP. mmPred introduces a dual-domain historical motion representation to guide the generation process, combining a Time-domain Pose Refinement (TPR) branch for learning fine-grained details and a Frequency-domain Dominant Motion (FDM) branch for capturing global motion trends and suppressing frame-level inconsistency. Furthermore, we design a Global Skeleton-relational Transformer (GST) as the diffusion backbone to model global inter-joint cooperation, enabling corrupted joints to dynamically aggregate information from others. Extensive experiments show that mmPred achieves state-of-the-art performance, outperforming existing methods by 8.6% on mmBody and 22% on mm-Fi.

==> sec/0_abstract.tex <==
\begin{abstract}

Existing Human Motion Prediction (HMP) relying on RGB- videos and MoCap annotation is sensitive to lighting conditions and raises privacy concerns, hindering its real-world applications such as firefighting and elderly care. Motivated by the robustness and privacy-preserving nature of millimeter-wave (mmWave) radar, we introduce radar as a novel sensing modality for HMP for the first time.
% In contrast, RF-based sensor commercial millimeter-wave (mmWave) radar offers a deployable alternative due to its robustness in adverse environments and privacy-preserving nature. Motivated by this, we introduce radar-based HMP, a novel task that predicts future human motion from historical mmWave radar data, such as point clouds (PCs). 
However, commercial mmWave radar suffers from limited resolution and multipath effects, resulting in sparse and noisy point clouds (PCs). Additionally, the radar signal is temporally inconsistent, with frequent keypoint mis-detections across frames, leading to unstable historical pose sequences. These issues pose significant challenges for accurate and coherent motion prediction.
%to motion modeling and producing realistic future motions.
% However, the mmWave radar has a limited resolution with severe noise, leading to challenges for accurate HMP. Specifically, occasional misdetections of body parts introduce temporal inconsistencies and pose instability, leading to unrealistic or anatomically implausible motion prediction. 
To address these challenges, we propose mmPred, a diffusion-based HMP framework for incorporating noisy radar inputs.
To mitigate the temporal inconsistency caused by intermittent body part miss-detection, we introduce the Frequency-domain Dominant Motion (FDM) module to directly extract historical motion representations in the frequency domain. By modeling the global temporal evolution of radar PCs, FDM captures dominant trend/velocity patterns that are robust to frame-level noise and provides a stable condition for the diffusion process. 
To further enhance motion realism under keypoint miss-detection, we propose a novel backbone, Global Skeleton Transformer (GST), to model joint-wise cooperation during diffusion. By modeling the skeleton as a fully connected structure, GST allows miss-detected joints to dynamically aggregate information from related ones, enabling coherent full-body motion.
% To extract more consistent velocity patterns, mmPred focuses on the most dominant motion in the frequency domain, predicting the historical pose sequence as the diffusion condition. 
% To further improve the motion realism, we propose a novel Transformer-based diffusion architecture for enhancing joint-wise correlation learning. 
Extensive experiments demonstrate mmPred outperforms the RGB-based baseline by 23\% under the adverse-environmental dataset mmBody, and surpasses the existing radar-based method by 22\% on the mm-Fi dataset.


% Due to limited spatial resolution, the point cloud provides sparse coverage near joint locations, often leading to keypoint miss-detection. The multipath effect of RF signals further causes temporal inconsistency, where body reflections fluctuate across consecutive frames. These spatiotemporal inconsistencies pose a key challenge for extracting coherent motion patterns and modeling future dynamics. 

%

% 
% \footnote[1]{The project page of pred is .}
\end{abstract}

% We propose to leverage mmWave radar as a low-cost alternative, which enables HMP in darkness and occlusion. However, the mmWave radar has a limited resolution with severe noise, making it hard to extract historical human motion trends.  Therefore, we propose a novel diffusion-based HMP framework, called mmPred. Two key designs are proposed by mmPred: (1) We jointly extract historical motion information in the time-frequency domain, alleviating the temporal inconsistency of radar point clouds. (2) We propose a novel spatial-temporal transformer for improving correlation between joints, which can infer mis-detected joints from other detected ones. Extensive experiments show mmPred outperforms the RGB-based method by 23\% under adverse environments and outperforms the state-of-the-art motion predictor by 22\% on mm-Fi. 

 % temporal inconsistency of radar PCs, 

% temporal inconsisteny

% temporal coherence, radar-specific, 
% feature-level flow module, 

% Human motion prediction (HMP) aims to forecast future human poses from historical motion and plays a critical role in applications such as human–robot interaction and autonomous systems. Existing HMP methods typically rely on optic-based sensors (e.g., RGB cameras) or motion capture (MoCap) systems to obtain historical poses. However, MoCap systems are costly and impractical for deployment, while cameras are vulnerable to adverse environmental conditions and raise privacy concerns. In contrast, commercial millimeter-wave (mmWave) radars offer a deployable alternative due to their robustness in challenging environments and inherent privacy-preserving nature. Motivated by this, we introduce radar-based HMP, a novel task that predicts future human motion from historical mmWave radar data, such as point clouds (PCs). Unlike optical sensors, mmWave radars provide lower spatial resolution and yield noisy, sparse PCs, posing unique challenges for motion prediction. First, radar signals are temporally inconsistent, which we address by modeling the entire motion sequence holistically in the frequency domain to extract dominant motion trends. Second, radar PCs often suffer from joint miss-detection. To address this, we explicitly model the global joint relationships, enabling the network to capture inter-joint cooperation and compensate for missing observations. To this end, we propose mmPred, a diffusion-based framework that incorporates both temporal and spatial priors for robust radar-based motion prediction. Extensive experiments show that mmPred outperforms an RGB-based baseline by 23\% under adverse conditions and surpasses the state-of-the-art radar-based method by 22\% on the mm-Fi dataset.


==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

\begin{figure}[!t]
\centering
\includegraphics[width=1.\linewidth]{sec/effect4.pdf}
\caption{(Left) Radar-based HMP under adverse environments (e.g., darkness). The model first estimates historical poses from raw mmWave radar PCs, then generates realistic future pose sequences.
(Right) t-SNE visualization of joint locations and velocities from predicted historical poses. We compare our frequency-domain prediction with the state-of-the-art pose estimator, PointTransformer~\cite{yang2023mm}.
Our method produces more structured and distinguishable velocity patterns across actions, while the time-domain baseline yields noisier velocity distributions.} 

% 没有建模 "global" joint interaction， （GCN），which might contain some valuable pattern, for example, the walking pattern requires non-local coordination of hand and feet. MOre over, radar has common miss-detection, hand or feet may be masked, rely on the global joint interction

% For example, when hand is miss-detect 

\label{Effect}
\end{figure}

% 频域可以捕捉更全局的信息（频域的好处），cite，
% 人在运动过程中有关节间的协调关系 cordination collaboration pattern，transformer 手和脚在走路的时候有协作
%% Global pose/skeleton relation Transformer. (对应for example 部分)

% ==================Background==================

\hc{3D Human Motion Prediction (HMP) aims to predict future human motion (i.e., human pose sequences) from observed historical poses, which plays an essential role in various applications such as human-robot interaction~\cite{gui2018teaching}, healthcare~\cite{troje2002decomposing}, and hazard prevention. 
Existing HMP works~\cite{chen2023humanmac, sun2024comusion} heavily rely on high-precision human pose history collected from Motion Capturing (MoCap) systems, which are typically expensive and impractical for most real-world deployments. Though combining optical sensors and estimation models like OpenPose~\cite{cao2019openpose} can capture historical pose sequences from RGB images, these methods have intrinsic limitations including low robustness against adverse environments (e.g., darkness and occlusion), and potentially raise privacy concerns for sensitive applications. 

% ==================Radar introduction==================

Radio frequency (RF) based millimeter-wave (mmWave) radar has emerged as a promising alternative to optical sensors due to its low price, portability, and scalable deployment~\cite{waldschmidt2021automotive}. 
Operated at 30-300 GHz~\cite{zhang2023survey}, they enable body imaging by learning the reflected signals, showing better robustness to darkness and occlusion.} Moreover, RF-sensors do not require appearance information, making them advantageous for privacy-preserving HMP applications. 
However, radars possess lower resolution than cameras due to bandwidth limitations, usually producing only hundreds of point clouds (PCs) with much noise. 
% \hc{This leads to difficulty in realizing accurate HMP. In particular, specular reflection and multipath effect~\cite{ding2024milliflow} of RF signals could frequently cause inconsistent sensing data}, e.g., miss-detection of body parts. 



% ==================Research Gap==================
In this paper, we propose a novel task: \textit{mmWave radar-based human motion prediction (mmHMP)}. 
%
% Unlike existing HMPs relying on high-precision MoCap data, radar-based HMP must predict future motion directly from noisy and incomplete mmWave radar PCs, making the task more challenging.
Unlike existing HMPs relying on MoCap data, mmHMP must predict future motion directly from radar PCs.
%
Prior image-based HMP methods~\cite{chao2017forecasting, wu2018real} first estimate 3D poses with pose estimators, then predict future motion from the estimated sequences. Following this paradigm, mmHMP typically relies on radar-specific pose estimators~\cite{chen2022mmbody, yang2023mm}.
%
However, these pose estimators struggle to handle temporal inconsistency issues of radar signals.
%
They are typically designed in the time domain, sensitive to occasional miss-detection in certain radar frames. % inconsistent signals and
%
As illustrated in Figure~\ref{Effect}, radar-estimated poses often suffer from jitter and vibration, which obscure important motion cues such as velocity.
%
Meanwhile, most existing HMP models, such as SPGSN~\cite{li2022skeleton}, adopt graph-based architectures to directly encode historical pose sequences. However, under jittery history and occasional keypoint miss-detection, these models are difficult to learn correct joint correlations or make realistic future predictions. 


% This paper introduces a novel task: human motion prediction (HMP) from mmWave radar. Unlike conventional HMP using ground-truth (GT) MoCap poses, radar-based HMP must extract spatial-temporal information directly from noisy and incomplete radar sensor data (e.g., PCs), making the task significantly more challenging.
% %
% Several attempts leverage RGB images for HMP~\cite{chao2017forecasting, wu2018real}. They first estimate historical human poses through pretrained image-based 3D pose estimator as preprocessing, and fed the predicted the pose sequences to HMP algorithms. 
% %
% Following such paradigm, radar-based HMP necessitate radar-based pose estimators~\cite{chen2022mmbody, yang2023mm, xue2021mmmesh, an2022fast, an2021mars} to reconstruct 3D poses. 
% %
% % Since radar PCs are sparse and do not explicitly contain human keypoints, existing PCs based HMPthese methods necessitate radar-based pose estimators~\cite{chen2022mmbody, yang2023mm, xue2021mmmesh, an2022fast, an2021mars} to estimate historical poses from PCs. 
% %
% Nevertheless, existing pose estimators are typically formulated in the time domain. The frame-by-frame approach is easily affected by noise or missing body parts in individual radar frames.
% %
% As shown in Figure~\ref{dual-ablation}(b), the estimated poses exhibit more jitter and vibration than RGB-estimated poses, obscuring critical motion cues such as velocity, as in Figure~\ref{Effect}. 
% %
% Moreover, most existing methods leverage Graph-based or VAE-based network architectures~\cite{yuan2020dlow, li2022skeleton, zhong2022spatio} to encode historical pose sequences directly. 
% %
% However, these encoders cannot robustly model joint interactions under noise.
% %
% When occasional mis-detection happens, the vibrating historical poses can lead to unrealistic future motion.


% ==================Motivation==================
Diffusion models (DMs) have recently been adopted for HMP, and
% Beyond generative ability,
the progressive denoising process has also proven effective for handling motion noise~\cite{chen2023humanmac}.
Motivated by this, we propose mmPred, a diffusion-based framework tailored for mmHMP. 
% Specifically, we first ...
% Then,
% Lastly,
mmPred aims to address two key challenges:
%
(1) To mitigate the temporal inconsistency in radar signals, mmPred operates in the frequency domain, directly estimating the dominant motion trend using Discrete Cosine Transform (DCT) representations~\cite{khayam2003discrete}.
%
%Unlike time-domain pose estimators that process frame-by-frame temporally inconsistent observations, 
In particular, DCT encodes a unified representation for the entire historical pose sequence,
% ~\cite{yi2023frequency}, 
where global motion patterns (e.g., mean pose and velocity) are captured in low-frequency components, and temporal jitter is isolated in the high-frequency band.
%
This enables the model to focus on global motion dynamics rather than frame-level temporal variation.
%
To implement this, we introduce the Frequency-domain Dominant Motion (FDM) module, which learns global features from historical radar PCs and predicts the low-frequency motion representation.
As shown in Figure~\ref{Effect} and Figure~\ref{dual-ablation}, FDM reduces vibration and captures consistent velocity patterns compared to prior state-of-the-art radar-based estimators.
% ~\cite{yang2023mm}.
% Diffusion models (DMs) can learn data distributions~\cite{ho2020denoising, song2019generative} and generate realistic samples, which have recently been applied to HMP~\cite{chen2023humanmac, barquero2023belfusion}. 
% %
% Through progressive noise elimination, they also demonstrate good noise-handling capability~\cite{zhang2024rohm}.
% %
% Motivated by such capabilities, we introduce mmPred, a diffusion-based framework for radar-base HMP.
% %
% To address the temporal inconsistency of the radar signal, mmPred directly estimates the dominant historical motion trend in the frequency domain~\cite{khayam2003discrete}. 
% %
% In the frequency domain, the entire historical human poses are represented as a whole~\cite{yi2023frequency}. The major motion trend (e.g., mean pose and velocity, etc) is concentrated in the low-frequency components, while temporal jitter is separated as high-frequency noise.
% %
% Such capability enables focus on the most dominant motion rather than noise in individual frames. 
% %
% Therefore, we propose our first module, named Frequency-domain Dominant Motion (FDM), which learns the PC features from the whole historical radar PCs to predict the low-frequency domain motion representation. 
% %
% As presented in Figure~\ref{Effect} and Figure~\ref{dual-ablation}, our method demonstrates more velocity information and less motion vibration.
%
(2) Furthermore, to facilitate more realistic motion generation, we model the relations among body joints (i.e., whole-body coordination). 
%
For instance, hand–leg coordination is critical for generating plausible motions like walking and running~\cite{bianchi1998kinematic}. 
%
Such structural priors potentially improve robustness under keypoint miss-detection, by leveraging relational cues from neighboring joints.
%
Inspired by this, we propose the Global Skeleton-relational Transformer (GST) as our diffusion backbone. GST dynamically captures the whole-body joint-wise dependencies throughout the denoising process, enabling anatomically coherent motion generation. %treats each joint as an individual token and
%
% In the experiments, we observe that GST reduces limb-length variance and improves motion plausibility.

% This motivates diffusion-based HMP, mmPred, tailored for handling noisy radar PCs and generating realistic future human motions. 
%
% Different from recent works that use DMs for HMP~\cite{chen2023humanmac, barquero2023belfusion}, DM for radar-based HMP confronts challenges from the noise and miss-detection issues. 
%


% %
% Though DCT has been widely applied in conventional HMP to smooth future motion trajectories, it has rarely been explored to extract human motion features from the noisy radar modality.
%
%Meanwhile, we also incorporate Time-domain Pose Refining (TPR) to jointly provide time-domain motion information, both serving as the diffusion's condition. 

% ==================Contributions==================
In summary, the contributions are threefold. First, we proposed a novel diffusion-based HMP framework tailored for noisy and sparse mmWave radar PCS. To the best of our knowledge, mmPred is the first method for radar-based HMP. Second, we propose a dual-branch condition module to extract motion history from radar PCs, as well as a novel HMP network architecture. (3) Extensive experiments show our proposed methods outperform existing methods by 8.6\% on mmBody and 22\% on mm-fi, achieving state-of-the-art (SOTA). 




% The major challenge for radar-based human motion prediction lies in the noisy PCs. While 

% This paper proposes the first mmWave radar-based HMP task, which is more challenging than HMP since its performance is jointly determined by two sub-processe: pose estimation from historical radar PCs and HMP using the predicted poses. Existing HMP methods~\cite{li2022skeleton, chen2023humanmac, sun2024comusion, yuan2020dlow} are typically designed for high-precision MoCap historical poses, which cannot handle noisy radar PCs. A few research have touched on HMP from unreliable historical poses~\cite{saadatnejad2022generic}, by proposing an auxiliary pose refinement task. However, they simulate with Gaussian noise that is different from the radar sensor noise. Specifically, existing radar-based pose estimators~\cite{chen2022mmbody, yang2023mm, xue2021mmmesh, an2022fast, an2021mars} are easily affected by occasional miss-detection in individual frames, leading sudden joint vibration in Figure~\ref{dual-ablation}(b). 


% This paper proposes a novel task: mmWave radar-based HMP. In contrast to the conventional HMP task, it is more challenging to extract spatial-temporal information from noisy radar PCs than from ideal GT historical poses. Existing HMP methods~\cite{li2022skeleton, zhong2022spatio, chen2023humanmac, sun2024comusion, yuan2020dlow} are typically designed to accept high-precision MoCap historical poses directly. They rely on radar-based pose estimation methods~\cite{chen2022mmbody, yang2023mm, xue2021mmmesh, an2022fast, an2021mars} to estimate historical poses. However, these pose estimators are typically formulated in the time domain. The frame-by-frame approach is easily affected by noise or missing body parts in individual frames. As shown in Figure~\ref{dual-ablation}(b), radar-estimated poses are temporally more jittery and vibrating than RGB-estimated poses, losing critical temporal information such as velocity. Under such circumstances, it is challenging to generate realistic future motion from vibrating history. Moreover, existing methods directly leverage Multilayer Perceptron (MLP) or Graph-based network architectures~\cite{li2022skeleton, zhong2022spatio} to encode historical pose sequences. However, it is more challenging to model the interaction between joints when miss-detection could occasionally happen. {chen2023humanmac, sun2024comusion, }



% our task presents significant challenges in the following aspects: (1) there exists no direct spatial mapping from 
% %
% This paper introduces a novel task: human motion prediction (HMP) from mmWave radar. Unlike conventional HMP using ground-truth (GT) MoCap poses, radar-based HMP must extract spatial-temporal information directly from noisy and incomplete point clouds (PCs), making the task significantly more challenging. 
% %
% While existing HMP methods~\cite{li2022skeleton, zhong2022spatio, chen2023humanmac, sun2024comusion, yuan2020dlow} assume access to accurate MoCap inputs, radar-based systems require pose estimators~\cite{chen2022mmbody, yang2023mm, xue2021mmmesh, an2022fast, an2021mars} to reconstruct historical poses from PCs. 
% %
% However, these estimators typically operate in the time domain and process frames independently, making them vulnerable to frame-wise noise and body-part miss-detections. As shown in Figure~\ref{dual-ablation}(b), the resulting radar-based poses exhibit significant temporal jitter, obscuring critical motion cues such as velocity. 
% %
% This degradation in history directly limits the realism of future motion predictions. 
% %
% Moreover, common motion encoders based on MLPs or GCNs~\cite{li2022skeleton, zhong2022spatio} struggle to model joint interactions robustly when such miss-detections disrupt the assumed spatial structure. 






% Though the emergence of Diffusion Models (DMs)~\cite{chen2023humanmac, sun2024comusion} are proposed to generate smooth transition between history and future, the degradation in history can leads to future degradation. To capture spatial correlation between joints, existing methods typically rely on GCN architectures~\cite{li2022skeleton, zhong2022spatio}, using predefined adjacent matrix. However, radar miss-detection could lead to information loss of certain joints. \jq{The spatially joint-wise miss-detection making fixed-adjacency information less reliable ?. }


% a1, 一句， a2 3,4句，spatial 2句，





% can estimate the human motion distribution,

% To address the challenges of radar-based human motion prediction (HMP), we adopt a diffusion-based generative framework. Diffusion models are well-suited for modeling the uncertainty and multi-modality inherent in radar data. Moreover, they naturally produce smooth and realistic motion trajectories, which are crucial when the historical input is noisy or incomplete. However, standard diffusion models rely heavily on the quality of historical motion representations. In radar-based HMP, the historical poses are often noisy and temporally inconsistent due to radar-specific challenges such as miss-detection, occlusion, and sparsity. Therefore, a key motivation of our work is to enhance the quality of historical motion encoding, such that the diffusion-based predictor can operate on a more stable and informative representation space. To this end, we propose to leverage the Discrete Cosine Transform (DCT)—a classical tool in signal processing—to model human motion from noisy radar point clouds. While DCT has been widely applied in conventional HMP to smooth future motion trajectories, it has rarely been explored as a temporal encoder for noisy historical observations, especially in radar-based settings. DCT provides a coarse-to-fine decomposition of motion dynamics: it treats the entire pose sequence as a whole, encodes low-frequency components (FCs) to capture dominant global trends such as mean pose and velocity, and separates out high-frequency variations. This global perspective makes DCT particularly suitable for radar inputs, where local noise and occasional joint miss-detections are common. Based on this insight, we introduce a DCT-based temporal encoding module that takes as input the full sequence of historical radar point clouds, extracts motion features, and estimates dominant temporal components in the DCT domain. In Figure~\ref{Effect}, we further show that even higher-order velocity cues can be reliably captured under noisy radar conditions via low-dimensional DCT representations. To handle joint-level sparsity and miss-detections, we propose a joint-wise decoupling strategy, where feature extraction is independently conducted for each joint. This design prevents corrupted joint observations from interfering with others during both historical encoding and future prediction. Finally, we design a spatial transformer module to dynamically model inter-joint dependencies, enabling adaptive spatial reasoning that is robust to missing or unreliable input joints.



% Therefore, in this paper, we propose to leverage Discrete Cosine Transform (DCT), a common tool signal processing, to handle the noisy radar modality. Though widely applied to HMP, DCT is typically applied to generate smooth motion in the future, not directly learning temporal motion features from historical radar modality, particularly with noise and temporal inconsistency (i.e., miss-detection). From figure~\ref{Effect}, we show its unique coarse-to-fine representation of human motion. Specifically, DCT representation treat the entire historical poses as a whole, concentrates the major motion information (e.g., mean pose, mean velocity, etc) in the low-frequency components (FCs), and separates high-frequency details. Therefore, we propose our first module, which take in the entire historical radar PCs as input, and learn a human motion representation in the DCT domain. Specifically, the model considers the overall PCs flow, extracts the PC features, and directly estimates the most dominant motion (low FCs). In Figure 1, we show that in the DCT domain, higher-derivative velocity information can be learned more efficiently given noisy and inconsistent radar signals. Moreover, to mitigate the effect of occasional miss-detection of body parts, we propose a strategy to isolate the feature learning for different joints, both during historical pose estimation and during future prediction. In this way, the miss-detected joints will not affect the feature extraction of the detected ones. Then, during future prediction, we design a spatial transformer that can dynamically learn the correlation between different joints. Specifically, 

% To this end,  we design mmPred, a diffusion-based HMP directly take in mmWave radar PCs to predict future human motion. mmPred first designs a dual-branch architecture to extract history poses in the time-frequency domain. A frequency-domain dominant pose flow branch is proposed that takes all historical radar PCs and outputs the low FCs in the DCT domain to represent historical human motion. Alongside we incorporate a time-domain pose refining branch performs frame-wise pose estimation. Subsequently, we fuse the estimated pose sequences from the two branches as the guiding feature of the HMP diffusion model, which is also learned in the DCT domain. Specifically, we design a novel model architecture that learns an individual feature embedding for each joint, and use a spatial transformer~\cite{vaswani2017attention} for joint-wise correlation learning. 



% Existing radar-based pose estimators~\cite{chen2022mmbody, yang2023mm, xue2021mmmesh, an2022fast, an2021mars} are easily affected by sensor noise and miss-detection in individual frames, leading to pose vibration as in Figure 1. However, existing HMP methods are typically 

% Traditional HMP methods are typically GCN-based or VAE-based~\cite{yuan2020dlow}, producing either single prediction or overly diverse unrealistic predictions. The emergence of diffusion-based methods~\cite{chen2023humanmac, sun2024comusion} enhance the realism and accuracy. But these methods heavily rely on high-precision MoCap-based historical poses. 


% To handle the noisy and sparse radar PCs, existing radar-based pose estimators~\cite{chen2022mmbody, yang2023mm, xue2021mmmesh, an2022fast, an2021mars} employ strategies such as multi-frame aggregation for data augmentation or leverage human motion prior knowledge to reduce historical pose vibration~\cite{fan2024diffusion}. \textit{Nevertheless, 





% Existing methods~\cite{chen2022mmbody, yang2023mm} have demonstrated the ability to estimate human poses across historical radar frames, \hc{while they are highly sensitive to radar miss-detections, often resulting in jittery and unstable pose sequences.} To improve consistency of pose estimation, \hc{a few recent methods employ strategies such as multi-frame aggregation~\cite{xue2021mmmesh, an2022fast, an2021mars} for data augmentation or pose refinement based on historical motion priors~\cite{fan2024diffusion}.} \textit{Nevertheless, these approaches are typically formulated in the time domain. For example, the frame-by-frame approach lacks a global understanding of how PCs evolve over time} \hc{and coubd be easily affected by noise or missing body parts in individual frames. As shown in Figure 1, miss-detection causes sudden joint displacement between consecutive frames}, which results in wrong prediction of curcial motion properties of HMP such as joint velocity.

% p#3: 分层，挑战(radar-based 以及 humanMAC)， 和组件对应出来，
% p#4: motivation -> 组件，





% With xxxx capability, Diffusion models (DMs)~\cite{ho2020denoising, song2020denoising} have been widely applied to 
% motion generation tasks~\cite{tevet2022human} and motion denoising tasks~\cite{zhang2024rohm}.
% % By learning the human motion distribution, DMs are also applied to motion denoising~\cite{zhang2024rohm} through 
% DMs could xxx iteratively remove nosie, ... and ..., which benefits/facilitates/enhances.
% \hc{Motivated by such capability, we design mmPred, a diffusion-based HMP tailored for the mmWave radar modality. Different from existing HMP methods using ground-truth (GT)? historical poses, HMP using radar PCs confronts two key challenges: (1) extracting robust history? motion trend and consistent velocity information from noisy PCs under miss-detection cases?, and (2) minimizing pose jitters in future motion generation?. For the first challenge, we propose analyzing motion in the frequency domain, allowing us to consider the entire motion sequence as a whole? and to capture more consistent velocity patterns? (how), as shown in Figure 1. Furthermore, we enhance joint-wise correlation learning for handling the lost joint information when miss-detected, thus ensuring more consistent limb-length and reducing pose jitters. 
% }

% To this end, mmPred first designs a dual-branch architecture for extracting history poses directly from radar PCs. Alongside a time-domain pose refining branch performing frame-wise pose estimation, we propose a frequency-domain dominant pose flow branch that takes all historical radar PCs and outputs the human pose sequence in the Discrete Cosine Transform (DCT) domain. In Figure 1, we show that in the DCT domain, higher-derivative velocity information can be learned more efficiently given noisy and inconsistent radar signals. Subsequently, we fuse the estimated pose sequences from the two branches as the guiding feature of the HMP diffusion model, which is also learned in the DCT domain. Specifically, we design a novel model architecture that learns an individual feature embedding for each joint, and use a spatial transformer~\cite{vaswani2017attention} for joint-wise correlation learning. 




% HMP is more challenging as it requires more fine-grained spatial-temporal cues. It is intriguing to answer: can we use noisy radar PCs for HMP?

% To handle modality noise, existing methods concatenate multi-frame radar PCs for single-frame pose estimation. mmDiff further proposes to reduce pose vibration using the multi-frame predicted pose as a temporal motion prior. Other methods are proposed for HMP using unreliable pose observation, using additional motion refinement for handling simulated Gaussian noise. However, radar sensor noise is fundamentally different from the simulated methods, as we have no knowledge of when radar miss-detection happens.


% Recent advances like ~\cite{chen2022mmbody, yang2023mm} have demonstrated the capability of estimating human poses. Different from existing HMP using GT poses as history, HMP using mmWave radar PCs confronts two key challenges: (1) extracting consistent motion trends from noisy PCs that suffer from occasional miss-detection, and (2) generating realistic future human motion from vibrating history motion. 

% Extracting history motion information (including both position and velocity) from noisy historical radar PCs. Particularly, occasional mis-detection of body parts causes 

% Generating future human motion that is robust to historical motion jitter, defined by vibrating limb length, enhances motion realism. 



% However, HMP from noisy radar points is a more challenging task requiring stronger temporal motion cues, which confronts the following challenges:
% \begin{itemize}
%     \item Mis-detection of body parts: Due to specular interference and multi-path effects, radar PCs appear inconsistent within adjacent frames.

%     \item Vibrating pose sequences: Existing radar-based human perception methods~\cite{chen2022mmbody, yang2023mm} are majorly in time-domain, estimating keypoint locations from frame to frame. These methods predict incorrect joint location when mis-detected, which cause sudden joint displacement and significantly wrong velocity, as in Fig 1.
% \end{itemize}


% So, can we predict human motion from radar, using noisy and sparse radar PCs.  Recent advances have demonstrated its ability to reconstruct human skeletal and mesh poses using point clouds (PCs) for target detection. However, the detected PCs are typically sparse and noisy, with frequent misdetections and temporal discontinuities. These limitations result in a jittery and unreliable history, posing significant challenges for understanding motion behavior and predicting the future. We are inspired to answer: Can we predict human motion using mmWave radar PCs?





% is defined to first observe a sequence of historical human poses/skeletons and predicting future human motion. It is the innate ability of humans to understand behavior and interact with each other, and is crucial for human-machine interaction and various safety applications (e.g., fall detection or hazard prevention). Existing methods [ref] take the ground-truth (GT) pose sequences collected from motion-capture systems as the history observation. However, such a tedious system is infeasible to deploy for a real-world application, and human pose observation is usually derived from RGB-based pose estimators, such as OpenPose. These camera-based pose estimators are inherently dependent on good illumination and unobstructed views, and fail in adverse scenarios involving darkness, occlusions, and smoke. Furthermore, the deployment of visual sensors in healthcare settings also raises privacy concerns.

% 3D Human Motion Prediction (HMP) is defined as first observing a sequence of historical human motion (human pose/skeleton) and predicting future human motion. It is the innate ability of humans to understand behavior and interact with each other, which is also important for human-machine interaction and various safety applications (e.g., fall detection or hazard prevention). Existing approaches predominantly rely on camera-based sensing systems, which are inherently dependent on good illumination and unobstructed views. As shown in Figure~\ref{Effect}, their performance degrades significantly in scenarios involving darkness, occlusions, smoke, or clutter challenges, which frequently arise in both indoor and outdoor environments. The deployment of visual sensors in healthcare settings also raises privacy concerns.







% In this paper, we focus on a new task utilizing RF-vision to perform human motion prediction under adverse scenes. Different from mmBody and mmMesh, which predict keypoint location for the current frame, our task requires more of the history motion velocity information for future prediction. Specifically the challenge is:
% miss detection... 

% existing methods cause pose vibrating, loss information

% We propose 

% Different from existing HMP works, our task should extract motion information from noisy radar point clouds, is highly non-trivial, while GT history is already available. 

% The challenge of radar-based HMP is to perceive human history motion from noisy and sparse radar PCs. 

% In Figure 1, we observe that radar point clouds are noisy and sparse because of low resolution, and human body parts may occasionally be miss-detected. Specifically, the existing radar-based HPE network can estimate human pose history. To mitigate the noise problem, they either concatenate adjacent frames for data augmentation, or borrow lstm or transformer architecture, for better representation learning. though achieve good accuracy, However, they are in time domain as in figure 1, the velocity information is lost. 







% The problem is further exacerbated by existing motion predictors trained on smooth ground-truth (GT) poses from motion capture systems, making them highly sensitive to noise and fluctuations in radar-based inputs.
% Existing HMP methods like CoMusion and humanMAC leverage diffusion models to learn the human motion distribution, generating realistic future motion using history information as the condition. However, they are trained by GT motion observation, making them highly sensitive to noise and vibration in radar-estimated poses. Other methods, like DePosit and Refine, add Gaussian noise to the pose history and propose pose refinement before motion forecast. However, there still exists a domain gap between handling simulated Gaussian noise and real-world sensor noise in mmWave radar. 


% To address this problem, we propose the first mmWave radar-based motion predictor, mmPred, capable of predicting future human poses under adverse environments. We demonstrate the capability of mmPred in Figure~\ref{Effect}. It leverages Discrete Cosine Transform (DCT) and a Diffusion model (DM), two powerful tools to handle the noisy modality. The DCT is widely used in signal processing, transforming real-valued temporal signals into the frequency domain. For typically smooth and temporally correlated human motion sequences, DCT demonstrates effectiveness in suppressing high-frequency noise [ref]. We leverage the diffusion models, widely applied in vision generation tasks (e.g., image generation), to generate realistic future motion. Recent advances [ref] have also shown its capability in image and motion denoising, demonstrating the capability to handle noisy observations. We leverage the diffusion model to learn DCT-domain motion distribution, generating plausible future motion and ensuring stable motion transition, thereby mitigating the impact of radar-induced jitter and vibration.

% Different from motion predictors that accept GT history, extracting motion features from radar-estimated human motion faces two key challenges: (1) heavy joint vibration hinders its real moving trend, and (2) severely undetected joints are less reliable than other detected ones. For the first challenge, joint misdetections of certain frames produce incorrect joint locations, resulting in sudden and inaccurate joint displacement in consecutive frames. This causes huge pose vibration, blinding the true motion direction and the moving velocity. For the second challenge, we observe that hands and legs are more difficult to detect by RF signals, making their history motion less reliable than other body parts. To tackle the challenges, we first design a motion flow estimator in the frequency domain alongside the pose predictor in the time domain. We define motion flow as the lowest few DCT coefficients capturing only the basic and dominant moving information, such as moving direction and average moving velocity. It eliminates high-frequency motion acceleration that potentially causes vibration. Secondly, we separate the historical motion feature for different joints, so that misdetected joints will not affect the feature extraction of detected joints. Then we propose a spatial-temporal transformer as the diffusion model backbone for enhanced anatomical correlation among joints. This design enables the network to infer plausible joint trajectories even when observations are partially missing, leveraging inter-joint dependencies.



% Human pose estimation (HPE) has been a widely-studied computer vision task for predicting coordinates of human keypoints and generating human skeletons~\cite{andriluka20142d, martinez2017simple, zhou2023adapose}. It is a fundamental task for human-centered applications, such as augmented/virtual reality~\cite{mehta2017vnect, zhou2023metafi++, yang2022metafi}, rehabilitation~\cite{tao2020trajectory, ar2014computerized}, and human-robot interaction~\cite{gao2019dual,deng2023long}. Current HPE solutions mainly rely on RGB(D) cameras~\cite{chen2018cascaded, kocabas2020vibe}. Though demonstrating promising accuracy, camera-based pose estimators have intrinsic limitations under adverse environments, e.g., smoke, low illumination, and occlusion~\cite{wang2021human}. The privacy issue of cameras also hinders the viability of HPE in medical scenarios, e.g., rehabilitation systems in hospitals~\cite{an2022mri}.

% Overcoming limitations of camera-based HPE, Radio-Frequency vision (RF-vision) has attracted surging attention for human sensing. The emerging mmWave radar technology presents a promising and feasible solution for HPE due to its price, portability, and energy efficiency~\cite{waldschmidt2021automotive}. Operated at the frequencies of 30-300 GHz~\cite{zhang2023survey}, commercial mmWave radars transmit and receive RF signals that penetrate human targets and occlusions. Radar point clouds (PCs) are further extracted as the salient target detection via monitoring signals' characteristic changes~\cite{rao2017introduction, xue2021mmmesh}. Therefore, the extracted PCs are more robust to adverse environments~\cite{zhao2018through} and reveal little privacy~\cite{yang2023mm}, inspiring accurate and privacy-preserving HPE~\cite{li2020capturing, yang2023mm, an2022fast, xue2021mmmesh}. However, due to the bandwidth and hardware limitations~\cite{prabhakara2023high}, radar PCs are sparse with limited geometric information~\cite {an2022fast}, leading to huge difficulties in achieving HPE. The sparse PCs are noisy in two aspects: (1) mmWave radar has a lower spatial resolution, leading to PC dispersion throughout the target area accompanied by ghost points caused by multi-path effect~\cite{sun20213drimr, prabhakara2023high}; (2) signal's specular reflection and interference~\cite{chen2022mmbody, bansal2020pointillism} further cause inconsistent sensing data, leading to occasional miss-detection of human parts.



% To deal with sparse and noisy mmWave PCs, existing solutions mainly rely on kinds of data augmentations, e.g., multi-frame aggregation to enhance PC resolution~\cite{an2022fast, xue2021mmmesh}. For the feature extractor, they directly borrow Long Short-Term Memory (LSTM)~\cite{xue2021mmmesh} or transformer-based architectures~\cite{chen2022mmbody, yang2023mm} from existing RGB(D) HPE methods. However, these feature encoders are tailored for visual and language modalities, which struggle to handle noisy and inconsistent radar PCs~\cite{qi2020analyzing}. As shown in Figure~\ref{Effect} (right), the existing SOTA solution~\cite{fan2021point} still suffers from pose vibration and severe drift, achieving undesirable performance.

% Denoising Diffusion Probabilistic Models (DDPMs)~\cite{ho2020denoising, song2020denoising}, also known as diffusion models, have demonstrated superior performance in various generative tasks, such as image generation and image restoration~\cite{hu2022global, zhu2023conditional, gong2023diffpose}. Diffusion models perform progressive noise elimination, transferring noisy distribution into desired target distribution~\cite{song2019generative}. Inspired by such capability, we aim to mitigate the noise of mmWave HPE, which motivates mmDiff, a diffusion-based pose estimator tailored for noisy radar PCs. Different from existing diffusion-based HPE using RGB(D), HPE using mmWave PCs confronts two key challenges: (1) extracting robust features from noisy PCs where miss-detection of human bodies may happen, and (2) overcoming signal inconsistency for stable HPE. For the first challenge, we propose to isolate the feature extraction for different body joints, so that occasional miss-detection would not affect the feature extraction of detected joints. Extracting features directly from local PCs also improves the feature resolution. For the inconsistency issue, prior knowledge of human body structure and motion can reduce unreasonable cases, achieving consistent feature learning. As the human structure has a size constraint where limb-length should remain constant~\cite{chen2021anatomy}, the limb-length can be additionally estimated to prevent pose variance. Moreover, inspired by human motion continuity~\cite{ramakrishna2013tracking} that discourages abrupt human behavior changes, historical poses can be leveraged for pose generation refinement, minimizing pose vibration.


% To this end, mmDiff first designs a conditional diffusion model capable of injecting radar information as the guiding conditions. Four modules are designed to extract clean and consistent information from radar point clouds: (1) Global radar context is proposed to isolate the globally extracted features for different human joints using a transformer~\cite{vaswani2017attention}, which generates more robust joint-wise features to handle miss-detection. (2) Local radar context is proposed to extract local features around body joints with a local transformer, which performs point-level attention for higher resolution. (3) Structural human limb-length consistency is proposed to extract human limb-length as consistent patterns, which reduce limb-length variance. (4) Temporal motion consistency is proposed to learn smooth motion patterns from historical estimated poses, which avoid pose vibration. Experiments have shown a significant improvement in pose estimation accuracy using mmDiff compared to the state-of-the-art models. Meanwhile, the generated poses demonstrate comparable structural and motion stability, validating the effectiveness of our designed conditional modules. 



% In summary, our contributions are three-fold. First, we propose a novel diffusion-based HPE framework with sparse and noisy mmWave radar PCs. To the best of our knowledge, mmDiff is the first diffusion-based paradigm for mmWave radar-based HPE. Second, four modules are proposed to extract robust representations from the noisy and inconsistent radar PCs considering global radar context, local radar context, structural limb-length consistency, and temporal motion consistency, used as the conditions to guide the diffusion process. Finally, extensive experiments show our approach achieves state-of-the-art performance on two public datasets: mmBody~\cite{chen2022mmbody} and mm-Fi~\cite{yang2023mm}. 


% This paper introduces a novel task: human motion prediction (HMP) directly using noisy radar PCs.
% %
% Existing HMP methods~\cite{yuan2020dlow,li2022skeleton, zhong2022spatio} are typically designed to accept high-precision MoCap historical poses. 
% %
% However, since sparse radar PCs contain little geometry information about human keypoints, these methods rely on radar-based pose estimators~\cite{chen2022mmbody, yang2023mm, xue2021mmmesh, an2022fast, an2021mars} to estimate historical poses. 

==> sec/1_intro1.tex <==
\section{Introduction}
\label{sec:introduction}

\begin{figure}[!t]
\centering
\includegraphics[width=1.\linewidth]{sec/effect4.pdf}
\caption{(Left) mmWave radar-based HMP under adverse environments (e.g., darkness).
(Right) t-SNE visualization of joint locations and velocities from predicted historical poses. We compare our frequency-domain prediction with the SOTA pose estimator~\cite{yang2023mm}.
Our method produces more distinguishable velocity patterns across actions, while the time-domain estimator yields noisier velocity distributions.} 

% 没有建模 "global" joint interaction （GCN），which might contain some valuable pattern, for example, the walking pattern requires non-local coordination of hand and feet. Moreover, radar has common miss-detection, hand or feet may be masked, relying on the global joint interction

% For example, when hand is miss-detect 

\label{Effect}
\end{figure}

% 频域可以捕捉更全局的信息（频域的好处），cite，
% 人在运动过程中有关节间的协调关系 cordination collaboration pattern，transformer 手和脚在走路的时候有协作
%% Global pose/skeleton relation Transformer. (对应for example 部分)

% ==================Background==================

3D Human Motion Prediction (HMP) aims to predict future human motion (i.e., human pose sequences) from observed historical poses, which plays an essential role in various applications such as human-robot interaction~\cite{gui2018teaching}, healthcare~\cite{troje2002decomposing}, and hazard prevention~\cite{yan2017development}. 
Existing HMP works~\cite{chen2023humanmac, sun2024comusion} heavily rely on high-precision human pose history collected from multi-view RGBD MoCap systems, which are typically expensive and impractical for most real-world deployments. Although some work~\cite{cao2017realtime} attempts to use single-view RGB images, these methods struggle under adverse environmental conditions (e.g., darkness, occlusion). Moreover, RGB-based approaches raise privacy concerns for sensitive scenarios such as elderly care. %optical sensors and

% ==================Radar introduction==================

Millimeter-wave (mmWave) radar has emerged as a promising alternative for human sensing due to its low price, portability, and scalable deployment~\cite{waldschmidt2021automotive}. 
As mmWave radar operates in the 30-300 GHz frequency range, its signals can penetrate visual obscurants such as smoke and function reliably regardless of lighting conditions~\cite{zhang2023survey}. Additionally, its limited spatial resolution naturally preserves privacy, making it suitable for HMP in indoor environments.
However, this also means that the resulting radar point clouds(PCs) are sparse due to limited spatial resolution~\cite{prabhakara2023high,rao2017introduction}. Radar PCs are also noisy due to "ghost" points caused by multipath effects~\cite{sun20213drimr}. These issues make it challenging to capture fine-grained motion from radar PCs. Moreover, intermittent miss-detection often occurs due to specular reflections~\cite{ding2024milliflow}, where only a subset of body parts reflect signals and others deflect signals away. Such temporal inconsistency severely obscures coherent keypoint trajectories for motion understanding.
%Such temporal inconsistency severely obscures coherent keypoint trajectories for motion understanding.

% This causes coarse geometric structure of the human body, making fine-grained historical motion modeling difficult. Moreover, due to specular reflections of RF signals~\cite{ding2024milliflow}, only a subset of body parts reflect signals while others are deflected and go undetected, leading to intermittent miss-detection over time. Such temporal inconsistency severely obscures coherent keypoint trajectories for motion understanding.

% However, radars possess lower resolution than cameras due to bandwidth limitations, usually producing only hundreds of point clouds (PCs) with much noise. 
% This leads to difficulty in realizing accurate HMP. In particular, specular reflection and multipath effect~\cite{ding2024milliflow} of RF signals could frequently cause inconsistent sensing data, e.g., miss-detection of body parts. 






% ==================Research Gap==================
These signal-level limitations directly degrade the quality of historical motion representation, which is critical for accurate future prediction. When conventional radar-based pose estimators~\cite{chen2022mmbody, yang2023mm} are applied frame-by-frame to extract historical human poses, PC sparsity and occasional miss-detection often lead to severe jitter, twisted body structures, and temporal inconsistency~\cite{fan2024diffusion}. As illustrated in Figure~\ref{Effect}, such jittery pose sequences obscure critical motion cues, particularly joint velocity, making it difficult for downstream HMP models to infer temporal motion intent. In contrast, existing HMP methods~\cite{martinez2017human, zhong2022spatio}, such as SPGSN~\cite{li2022skeleton}, typically assume ideal historical observations from MoCap systems. They simply apply low-pass filtering directly on radar-estimated poses, which is insufficient for handling severe structural distortions and often produces misleading velocity trends. To model spatial joint relationships, they directly apply graph-based encoders on vibrating and twisted radar poses, often producing future motion with inconsistent or anatomically implausible inter-joint cooperation. 


% In this paper, we propose a novel task: \textit{mmWave radar-based human motion prediction (HMP)}. 
% %
% % Unlike existing HMPs relying on high-precision MoCap data, radar-based HMP must predict future motion directly from noisy and incomplete mmWave radar PCs, making the task more challenging.
% Unlike existing HMP methods using MoCap-based historical inputs, radar-based HMP requires estimating motion representations directly from sparse and noisy radar PCs.
% %
% Prior image-based HMP methods~\cite{chao2017forecasting, wu2018real} typically estimate 3D poses with image-based pose estimators~\cite{rombach2022high}, then predict future motion from the estimated sequences. Following this paradigm, radar-based HMP should rely on radar-specific pose estimators~\cite{chen2022mmbody, yang2023mm}.
% %
% However, these pose estimators struggle to handle temporal inconsistency issues of radar signals.
% %
% They are typically designed in the time domain, sensitive to occasional miss-detection in certain radar frames. % inconsistent signals and
% %
% As illustrated in Figure~\ref{dual-ablation}(b) and Figure~\ref{Effect}, radar-estimated poses often suffer from jitter and vibration, which obscure important motion cues such as velocity (i.e., noisy velocity distribution).
% %
% Meanwhile, most existing HMP models, such as SPGSN~\cite{li2022skeleton}, adopt graph-based encoder-decoder architectures to model historical pose sequences. However, under occasional miss-detection of certain body parts, these models struggle to learn reliable joint correlations, making it challenging to generate realistic and anatomically plausible future motions.
% %~\cite{yuan2020dlow, zhong2022spatio}


% ==================Motivation==================
Diffusion model (DMs) is a class of probabilistic generative models showing great potential in human motion generation~\cite{tevet2022human}. By learning the data distribution from realistic human motion samples, DMs can perform progressive noise elimination to generate temporally coherent motion sequences even from noisy initializations~\cite{zhang2024rohm}. 
% Diffusion models (DMs) can generate realistic human motion and perform motion denoising~\cite{zhang2024rohm} by modeling the complex human motion distribution.
%
Motivated by such capability, we propose mmPred, a diffusion-based HMP framework tailored for noisy radar PCs. 
%
Unlike existing diffusion-based HMP~\cite{chen2023humanmac} using MoCap history, mmPred aims to address two key challenges caused by noisy radar PCs:
%
(1) To address temporal inconsistency caused by occasional miss-detection, mmPred directly extracts historical motion in the frequency domain, estimating the Discrete Cosine Transform (DCT) components to capture the dominant motion trend.
%
%Unlike time-domain pose estimators that process frame-by-frame temporally inconsistent observations, 
In particular, DCT offers a unified representation for the entire pose history, where global motion patterns (e.g., mean pose with stable velocity) are captured in low-frequency components, and temporal jitter is isolated in the high-frequency band.
%
This enables the model to focus on global PC evolution rather than frame-level temporal variation, capturing global human motion dynamics.
%
As shown in Figure~\ref{Effect}, our frequency-domain design captures more consistent velocity patterns compared to prior state-of-the-art radar-based estimators. 
%
(2) To enable more realistic motion generation under occasional keypoint miss-detection, mmPred incorporates joint-wise self-attention within the diffusion framework to dynamically model global joint cooperation.
%
This is inspired by natural motions like walking or running, which inherently involve synchronized movement across distant joints, such as the hands and legs.
%
By capturing such structural prior knowledge, the model can infer missing keypoints by attending to correlated joints, thereby improving robustness.
%


To this end, mmPred first adopts a more robust dual-domain design to estimate historical human motion dynamics from radar PCs. A Time-domain Pose Refining (TPR) module is proposed to extract frame-wise human poses in a coarse-to-fine manner. More importantly, we introduce the Frequency-domain Dominant Motion (FDM) module, which learns global PC features from all historical radar PCs and predicts the frequency-domain motion representation. Using dual-domain historical motion representation as the condition, mmPred further designs a frequency-domain diffusion model for future motion prediction. To facilitate joint-wise co-operation learning, we propose the Global Skeleton-relational Transformer (GST) as our diffusion backbone. GST captures both spatial-temporal correlation along the joint and frequency dimension, respectively, enabling anatomically and temporally coherent motion generation. In summary, the contributions are threefold: (1) We proposed a novel diffusion-based HMP framework tailored for noisy and sparse mmWave radar PCS. To the best of our knowledge, mmPred is the first method for radar-based HMP. (2) We propose a dual-branch condition module to extract motion history from radar PCs, as well as a novel HMP network architecture. (3) Extensive experiments show our proposed methods outperform existing methods by 8.6\% on mmBody and 22\% on mm-fi, achieving state-of-the-art. 


% Diffusion models (DMs) can learn data distributions~\cite{ho2020denoising, song2019generative} and generate realistic samples, which have recently been applied to HMP~\cite{chen2023humanmac, barquero2023belfusion}. 
% %
% Through progressive noise elimination, they also demonstrate good noise-handling capability~\cite{zhang2024rohm}.
% %
% Motivated by such capabilities, we introduce mmPred, a diffusion-based framework for radar-base HMP.
% %
% To address the temporal inconsistency of the radar signal, mmPred directly estimates the dominant historical motion trend in the frequency domain~\cite{khayam2003discrete}. 
% %
% In the frequency domain, the entire historical human poses are represented as a whole~\cite{yi2023frequency}. The major motion trend (e.g., mean pose and velocity, etc) is concentrated in the low-frequency components, while temporal jitter is separated as high-frequency noise.
% %
% Such capability enables focus on the most dominant motion rather than noise in individual frames. 
% %
% Therefore, we propose our first module, named Frequency-domain Dominant Motion (FDM), which learns the PC features from the whole historical radar PCs to predict the low-frequency domain motion representation. 
% %
% As presented in Figure~\ref{Effect} and Figure~\ref{dual-ablation}, our method demonstrates more velocity information and less motion vibration.
%


%treats each joint as an individual token and
%
% In the experiments, we observe that GST reduces limb-length variance and improves motion plausibility.

% This motivates diffusion-based HMP, mmPred, tailored for handling noisy radar PCs and generating realistic future human motions. 
%
% Different from recent works that use DMs for HMP~\cite{chen2023humanmac, barquero2023belfusion}, DM for radar-based HMP confronts challenges from the noise and miss-detection issues. 
%


% %
% Though DCT has been widely applied in conventional HMP to smooth future motion trajectories, it has rarely been explored to extract human motion features from the noisy radar modality.
%
%Meanwhile, we also incorporate Time-domain Pose Refining (TPR) to jointly provide time-domain motion information, both serving as the diffusion's condition. 

% ==================Contributions==================


%These signal-level limitations directly impair the quality of historical motion representation, which is critical for accurate future prediction. Using existing radar-based pose estimators~\cite{chen2022mmbody, yang2023mm} to extract historical human poses frame-by-frame, PC sparsity and miss-detection often result in severe jitter, twisted structures, and temporal inconsistency. Such disturbances obscure essential motion cues (i.e., joint coordination and velocity), as shown in Figure~\ref{Effect}. When the model is conditioned on corrupted histories, it becomes difficult to capture temporal dynamics and motion intent. On the other hand, existing HMP pipelines often assume ideal historical observations obtained from high-fidelity MoCap or RGB-based pose estimators. To model temporal smoothness, most existing HMP models, such as SPGSN~\cite{li2022skeleton}, directly apply low-pass filters on radar-estimated history, often incapable to handle severe twisting and producing incorrect motion intent and velocity. To capture spatial joint correlation, they directly adopt graph-based encoder-decoder architectures to encode the history with twisted pose structures, often leading to implausible or anatomically inconsistent predictions.


==> sec/3_methodology.tex <==

\section{Methodology}
\label{sec:methodology}




%-------------------------------------------------------------------------
Our proposed mmWave radar-based HMP task inputs historical $H$ frames of radar PCs and predicts future $F$ frames of human poses. We denote the radar PCs as $R^{1:H}=\{R^i \in \mathbb{R}^{N\times6}\}^{H}_{i=1}$, which are robust inputs under adverse environments. Each historical frame contains $N$ points, and each point has three Cartesian coordinates $\{x,y,z\}$ and three features $\{v,E,A\}$ representing velocity, energy, and amplitude. The predicted future pose sequences are denoted as $\hat{x}^{H+1:H+F}=\{x^i\}^{H+F}_{i=H+1}$. Different from the existing 3D HMP task, which takes in historical ground-truth (GT) human poses $x^{1:H}=\{x^i \in \mathbb{R}^{J\times3}\}^{H}_{i=1}$, where $J$ denotes the number of body joints, our task involves estimating historical poses from radar data. Specifically, we predict $H$ frames of historical poses $\tilde{x}^{1:H}=\{\tilde{x}^i \in \mathbb{R}^{J\times3}\}^{H}_{i=1}$ and use them for future motion prediction. Given that historical radar PCs contain substantial noise, our task is fundamentally more challenging.



% The system architecture is presented in Figure~\ref{system architecture}. It first learns to extract historical motion information from radar PCs, and subsequently, a frequency-domain diffusion model learns to generate the complete pose sequence (with $H+F$ frames) using the extracted information. In the following sections, we start with a preliminary overview of how human motion is represented and how diffusion models can generate human motion in the frequency domain. Then, in Section~\ref{dual-branch}, we discuss how the dual-branch architecture is designed to extract robust and consistent historical motion information from noisy radar PCs. Finally, in Section~\ref{spatial-temporal}, we propose a spatial-temporal diffusion network architecture, using inter-joint dependency to handle occasional mis-detection of human joints.


%-------------------------------------------------------------------------
\subsection{Preliminary}
\label{preliminary}

\subsubsection{DCT-domain Human Motion Representation.} The \textit{Discrete Cosine Transform (DCT)}, a widely-used signal processing tool, can transform time-domain human pose sequences into frequency-domain coefficients, offering a compact representation.
Let $\mathbf{x}^{1:T} \in \mathbb{R}^{T \times 3J}$ be a time-domain pose sequence of ($T$) frames, and let $\mathbf{X}^{1:N} \in \mathbb{R}^{N \times 3J}$ denote the truncated DCT representation ($N \le T $), as an output of DCT. The type-II orthonormal DCT is defined as:
\begin{equation}
\mathbf{X}^{1:N} = \mathcal{F}_{DCT}(\mathbf{x}^{1:T}) = \mathbf{D} \mathbf{x}^{1:T}
\label{eq:dct_matrix},
\end{equation}
where \( \mathbf{D} \in \mathbb{R}^{N \times T} \) is the DCT basis matrix with entries:
\begin{equation}
\begin{aligned}
    D_{k,t} = \alpha_k \cdot \cos\left[ \frac{\pi}{T} \left(t + \tfrac{1}{2} \right) (k-1) \right],\\
    \alpha_k = \sqrt{\tfrac{1}{T}}, k = 1; \alpha_k = \sqrt{\tfrac{2}{T}}, k > 1.
\end{aligned}
\end{equation}
The inverse DCT reconstructs the time-domain pose sequences via:
\begin{equation}
\hat{\mathbf{x}}^{1:T} = \mathcal{F}_{iDCT}(\mathbf{X}^{1:N}) = \mathbf{D}^\top \mathbf{X}^{1:N}.
\label{eq:idct_matrix}
\end{equation}
In the frequency domain, human motion is represented holistically rather than frame-by-frame as in the time domain. Moreover, DCT coefficients decompose motion in a coarse-to-fine manner: dominant motion trends with the majority of the signal energy are concentrated in the low-frequency components, while fine-grained details and jitter are captured in the high-frequency bands. This property makes DCT particularly suitable for radar-based motion analysis, where signals are affected by temporal inconsistency, such as frame-wise miss-detection.


\subsubsection{DCT-domain Diffusion Model for HMP}

DMs can model realistic human motion distribution and have recently been popular in various human motion generative tasks, e.g., text-to-motion generation~\cite{tevet2022human}. Conditioned on semantic text, DMs generate diverse and realistic human motion from random noise initialization, through a progressive denoising process. Extended to HMP, DMs leverage historical motion information as a condition to inpaint the missing future parts, generating smooth motion transitions that match the human motion distribution. For HMP under the noisy radar modality, where historical poses often exhibit jitter and temporal inconsistency, we design a diffusion-based framework operating in the DCT domain. It focuses on learning low-frequency motion components while suppressing high-frequency jitters.

Given the GT time-domain pose sequence $\mathbf{x}^{1:(H+F)} \in \mathbb{R}^{(H+F) \times 3J}$ (both history and future), we apply the DCT transformation $\mathcal{F}_{DCT}^1$ using basis $\mathbf{D}_1 \in \mathbb{R}^{N_1 \times (H+F)}$ to obtain its DCT-domain representation $X^{1:N_1}$. The diffusion model consists of two processes: a forward process that gradually adds noise and a reverse process that learns to invert. In the forward process, we start from the DCT-domain GT $X_0 = X^{1:N_1}$. For each diffusion step $k\in[0,..,K]$, we iteratively sample a noisier motion $X_k$ by adding Gaussian noise $\varepsilon \in \mathcal{N}(0, I)$:

\begin{equation}
    q\left(\mathbf{X}_k \mid \mathbf{X}_{k-1}\right) = \mathcal{N}\left(\mathbf{X}_k \mid \sqrt{1-\beta_k} \mathbf{X}_{k-1}, \beta_k \mathbf{I}\right),
\label{eq：forward}
\end{equation}
where $\beta_k$ is the scheduled noise scale. On the contrary, the reverse process starts from a noisy Gaussian initialization $\hat{\mathbf{X}}_K \in N(0,I)$ and progressively removes noise until $\hat{\mathbf{X}}_0$ is generated. A diffusion model, denoted as $\hat{\varepsilon}_\theta$, is trained to identify the motion noise $\hat{\varepsilon}_k$ within $\hat{\mathbf{X}}_k$, and remove it for cleaner motion $\hat{\mathbf{X}}_{k-1}$:

\begin{equation}
    \begin{aligned}
    \hat{\varepsilon}_k &= \hat{\varepsilon}_\theta(\hat{\mathbf{X}}_k, k,C),\\
    \hat{\mathbf{X}}_{k-1} &= (1-\beta_k)^{-1}(\hat{\mathbf{X}}_{k} - \beta_k\hat{\varepsilon}_k).
    \end{aligned}
\label{eq:diff23}
\end{equation}
To ensure the predicted future follows historical human behavior, we leverage the historical human pose sequences as the condition $C$ for guiding the diffusion model. Under our radar-based HMP setting, the historical pose sequences are produced from mmWave radar PCs $R^{1:H}$. In the subsequent section, we will discuss how to extract robust historical motion representation as reliable diffusion guidance.




\begin{figure}[!t]
\centering 
\includegraphics[width=1.\linewidth]{sec/dual-ablation1.pdf}
\caption{Comparison of historical pose estimation from radar PCs in the time domain and frequency domain. Colored poses are predictions; black poses are GTs. We zoom in on the hand area and use red arrows to mark the joint velocity (displacement of consecutive frames).}
\label{dual-ablation} 
\end{figure}




\subsection{Dual-Domain Historical Motion Estimation}
\label{dual-branch}
Accurate guidance for diffusion-based motion prediction relies on robust historical motion estimation—requiring both precise joint localization and a coherent motion trend. As shown in Figure~\ref{dual-ablation}, frame-wise miss-detections cause abrupt joint shifts, resulting in jitter and disrupted motion trends. To address this, we propose a dual-domain historical motion estimation approach: The Time-domain Pose Refining (TPR) module focuses on accurate joint locations, in a frame-by-frame and coarse-to-fine manner. Complementarily, the Frequency-domain Dominant Motion (FDM) module takes the entire radar sequence as input and predicts a DCT-domain motion representation, aiming to capture dominant and consistent motion trends.
%However, radar point clouds are noisy and temporally inconsistent;

\subsubsection{Time-domain Pose Refining (TPR).} 
% TPR reconstructs historical human poses from radar data by applying a pretrained pose estimator frame by frame, followed by a pretrained pose refiner to enhance spatial accuracy. 
For each frame $i \in [1, \dots, H]$, TPR employs a shared pretrained pose estimator~\cite{chen2022mmbody, yang2023mm}, denoted as $f_{\text{pose}}$, to predict 3D human poses from the single-frame radar point cloud $R^i$. However, occasional joint miss-detections may cause certain joints to deviate significantly from their true positions, resulting in twisted pose structures or jitter across frames. To mitigate this, we employ a pretrained diffusion-based refinement network~\cite{fan2024diffusion}, denoted as $f_{\text{refine}}$. It leverages prior knowledge such as limb-length consistency and adjacent-frame continuity to improve structural plausibility and temporal stability. Given the coarse output from $f_{\text{pose}}$, it produces refined pose estimates $\tilde{x}^i_{\text{time}}$ for each frame. Finally, we aggregate the refined poses from all $H$ frames as the TPR output:
\begin{equation}
    \begin{aligned}
    \tilde{x}_{\text{time}}^{i} &= f_{\text{refine}}(f_{\text{pose}}(R^i))\\
    \tilde{x}_{\text{time}}^{1:H} &= \{\tilde{x}_{\text{time}}^{1},\tilde{x}_{\text{time}}^{2},...,\tilde{x}_{\text{time}}^{H}\}^H_{i=1} 
    \end{aligned}
\end{equation}
% TPR reconstructs historical human poses from radar data by applying a pretrained pose estimator frame by frame, followed by a pretrained pose refiner to enhance spatial accuracy. For each frame $i \in [1, \dots, H]$, the TPR employs a shared pretrained pose estimator~\cite{chen2022mmbody,yang2023mm} $f_{\text{pose}}$, typically an encoder-decoder architecture, to predict 3D human poses from the single-frame radar PC $R^i$. The encoder commonly follows an anchor-based design to extract PC features: Firstly, a set of representative anchor points is first selected using Farthest Point Sampling (FPS), and local features around these anchors are aggregated as the anchor features. These anchor features are subsequently passed through a pose decoder to estimate the 3D joint positions. However, occasional joint miss-detections may cause certain joints to deviate significantly from their true positions, resulting in twisted pose structures or jitter across frames. 
% To mitigate this, we employ a pretrained pose diffusion-based refinement network~\cite{fan2024diffusion}, denoted as $f_{\text{refine}}$, to refine poses frame by frame. 
% which is  to learn structural priors such as limb-length consistency and temporal smoothness. It takes the coarse output from $f_{\text{pose}}$ and produces refined pose estimates $\tilde{x}^i_{time}$ that are more physically plausible and temporally stable. Finally, we aggregate historical $H$ frames of the refined poses as output:

% \begin{equation}
%     \begin{aligned}
%     \tilde{x}_{time}^{i} &= f_{refine}(f_{pose}(R^i))\\
%     \tilde{x}_{time}^{1:H} &= \{\tilde{x}_{time}^{1},\tilde{x}_{time}^{2},...,\tilde{x}_{time}^{H}\}^H_{i=1} 
%     \end{aligned}
% \end{equation}

% TPR operates in the time domain, focuses on accurate keypoint location.

% The module extracts the historical pose sequence in the time domain. It focuses on the most likely joint locations given the radar PC cues, to maximize the accuracy of detected joints. For each frame $i \in [1,.., H]$, it leverages a shared pretrained pose regressor $f_p$ to predict human poses such as P4Transformer~\cite{chen2022mmbody} or PointTransformer~\cite{yang2023mm}. Since mis-detection may happen to certain joints, they may deviate from the correct location and lead to pose twisting and vibration. So we adopt mmDiff~\cite{fan2021point}, denoted as $f_r$, a pretrained pose refiner for pose refinement. Specifically, it corrects twisted poses using prior knowledge such as limb-length constraints and reduces pose jittering using previous-frame poses. Finally, we aggregate historical $H$ frames of predicted poses as output:
% \begin{equation}
%     \begin{aligned}
%     \tilde{x}_p^{i} &= f_r(f_p(R^i))\\
%     \tilde{x}_p^{1:H} &= \{\tilde{x}_p^{1},\tilde{x}_p^{2},...,\tilde{x}_p^{H}\} 
%     \end{aligned}
% \end{equation}

 
\subsubsection{Frequency-domain Dominant Motion (FDM).} 
FDM directly outputs a compact DCT-domain representation, treating the entire historical motion sequence holistically. It takes all $R^{1:H}$ as input and predicts the DCT-domain motion representation, $\tilde{X}^{1:N_2}_{\text{freq}}\in \mathbb{R}^{N_2\times J \times 3}$, where $N_2$ denotes the number of selected coefficients (typically $N_2 = 3$ or $4$). These few coefficients capture the most dominant motion dynamics, allowing the model to focus on a robust and consistent motion trend. % such as mean pose and velocity, rather than noisy frame-wise variations
%As a result, the FDM produces temporally smooth and velocity-consistent motion representations. 
%Unlike the TPR branch that estimates keypoints frame-by-frame, the
%In the supplementary material, we further analyze the physical meaning of the first few DCT components and their effectiveness in suppressing radar noise and jitter.

As shown in Figure~\ref{system architecture}, we first utilize an anchor-based PC encoder $f_{\text{pc}}$ (structurally similar to the one in TPR but trainable) to extract features from all-historical-frame radar PCs $R^{1:H}$. Specifically, for each frame, we select $N'$ representative anchor points using Farthest Point Sampling (FPS). Each anchor feature encodes local spatial information from its neighborhood, aggregated into anchor features $F_{r}\in\mathbb{R}^{(H \times N') \times 1024}$. To further encode the motion evolution over time, we inject temporal positional information using an MLP that maps each anchor’s $(x, y, z, t)$ (where $t \in [1, H]$) to an embedding, serving as positional encoding. This encoding is then added to the corresponding anchor features.

However, these anchor features are extracted in the time domain, and directly applying DCT to them leads to unstable high-frequency coefficients due to noise and inconsistency in individual radar frames. Therefore, we adopt a cross-domain transformer $\Phi$ to dynamically project time-domain anchor features into frequency-domain joint motion features. We first zero-initialize a set of learnable joint template tokens $\bar{F}_j \in \mathbb{R}^{J \times 1024}$, one for each body joint. These are concatenated with the anchor features and jointly processed by $\Phi$:
\begin{equation}
    \begin{aligned}
        F_r &= f_{\text{pc}}(R^{1:H}),\\
        F'_r, F_j &= \Phi(F_r, \bar{F}_j).
    \end{aligned}   
\end{equation}
Within the transformer, each joint feature in $F_j$ dynamically aggregates information from the anchor tokens via self-attention, capturing its motion pattern from correlated anchor feature cues. The captured joint features $F_j$ are eventually decoded by an MLP-based motion decoder $f_{j}$ to produce the DCT-domain representation:
\begin{equation}
    \tilde{X}_{\text{freq}}^{1:N_1} = f_{j}(F_j).
\end{equation}


\subsection{Global Skeleton-Cooperative Future Prediction}

Occasional keypoint miss-detection may lead to unreliable feature representations for certain joints. While existing diffusion models~\cite{chen2023humanmac} encode all joints into a unified feature vector and apply self-attention solely along the temporal or frequency dimension. This design potentially injects noise from corrupted joints into the latent space. Therefore, we propose a new diffusion model architecture for radar-based HMP, which enhances global skeleton cooperation learning. In the following subsections, we first describe how to construct the condition embedding $C$ from dual domain historical motion. Then, we introduce the design of the Global Skeleton Transformer (GST).




% Existing diffusion models, such as HumanMAC~\cite{chen2023humanmac}, encode all joints into a unified feature representation and apply self-attention only along the temporal/frequency dimension. Unlike them, we 

% To address joint miss-detection, we first separate joint features by assigning each joint an independent embedding when encoding both the condition $C$ and diffusion input $X_k$. This prevents corrupted joints from affecting others and preserves individual motion characteristics. We then introduce the Global Skeleton Transformer (GST) to model joint-wise interactions. GST applies self-attention across all joints, enabling adaptive feature communication, where miss-detected joints can aggregate information from correlated ones.
% GST applies self-attention across all joints, enabling adaptive feature communication, where miss-detected joints can aggregate information from correlated ones.

% model to assign joint-wise importance based on spatial correlations. This mechanism helps refine features of miss-detected joints by aggregating cues from related joints, resulting in more robust and coherent representations.


% Due to keypoint miss-detection, certain joint information may be less reliable. To handle this, we propose to first isolate feature representation of different joint, preventing miss-detected joints from polluting others. (provide a unique feature representation for each joint, capturing their individual motion feature), both for conditional embedding and for the motion feature of $X_k$. 

% Then, the joint feature is aggregated in the GST model. Specifically, then, we propose the GST model to model the global copperation/correlation, considering all joints as correlated whole entity. 

% Within the GST, joint fetures can perform information communication between different joints, in a dynamic way to enlarge or reduce the weight of the feature. Through this process, miss-detected joint feature can aggregated information from neighboring detected ones, 

\subsubsection{Cross-Domain History Fusion} 

To guide the diffusion model, we fuse the time-domain $\tilde{x}_{time}^{1:H}$ and frequency-domain $\tilde{X}_{freq}^{1:N_2}$ into a conditional embedding $C$. Since the diffusion process operates in the frequency domain, we transform both inputs into frequency domain representations, $\tilde{X}_{\text{time}}^{1:N_1}$ and $\tilde{X}_{\text{freq}}^{1:N_1}$, with $N_1$ DCT coefficients corresponding to $H+F$ frames. The detailed preprocessing steps are provided in the Appendix.
% Firstly, $\tilde{x}_{time}^{1:H}$ is repeated-padded with its last frame $\tilde{x}_{time}^{H}$ for $F$ times and transformed to the DCT domain using $\mathcal{F}_{DCT}^{1}$:
% \begin{equation}
%     \tilde{X}_{time}^{1:N_1} = \mathcal{F}_{DCT}^{1}(pad(\tilde{x}_{time}^{1:H})).
% \end{equation}
% For the $\tilde{X}^{1:N_2}_{freq}$, we first apply $\mathcal{F}_{iDCT}^{2}$ to recover the time-domain sequence. Then we apply the same repeated-padding and DCT transformation:
% \begin{equation}
%     \tilde{X}_{freq}^{1:N_1} = \mathcal{F}_{DCT}^{1}(pad(\mathcal{F}_{iDCT}^{2}(\tilde{X}_{freq}^{1:N_2}))).
% \end{equation}
Then, both representations are reshaped into $J$ individual joint motion features of dimension $N_1 \times 3$, treating each joint independently. This joint-wise isolation preserves the distinct motion dynamics of each keypoint and prevents unreliable joints (i.e., caused by radar miss-detection) from affecting others. It also enables structured joint-wise processing in the subsequent diffusion stages. As an implementation, each joint feature is independently projected via two MLPs $f_1$ and $f_2$, and then fused by element-wise addition to obtain the final joint-wise conditional embedding $C\in\mathbb{R}^{J\times 384}$:
\begin{equation}
    C = f_1(\tilde{X}_{\text{time}}^{1:N_2}) + f_2(\tilde{X}_{\text{freq}}^{1:N_2}). 
\end{equation}



\subsubsection{Global Skeleton-Relational Transformer (GST).}
\label{spatial-temporal}

Existing transformer-based diffusion models typically overlook global cooperation between human joints during motion generation. They encode all joints into a unified representation and apply self-attention only along the temporal or frequency dimension. Such a design is vulnerable to joint miss-detection, where unreliable joints can degrade the quality of the latent features.
To address this, GST first isolates the feature representations of individual joints, preserving joint-specific motion information. Then, we introduce spatial self-attention to dynamically aggregate joint features, enabling global information exchange and enhancing robustness against noisy or missing keypoints.

GST designs two Transformers that separately model spatial and temporal dependencies of motion. As shown in Figure~\ref{system architecture}, the noisy motion of intermediate diffusion step $k$, $X_k \in \mathbb{R}^{N_1 \times J \times 3}$, is first projected to latent features $H_k \in \mathbb{R}^{N_1 \times J \times 384}$ by an MLP. This yields $N_1 \times J$ tokens, one for each joint at each frequency coefficient.
For spatial modeling, we reshape $H_k$ into $\mathbb{R}^{J \times (N_1 \times 384)}$, aggregating all frequency components into joint-specific tokens. These $J$ tokens are passed through a Skeleton Transformer (S-Transformer), where self-attention enables joint-wise interaction. This mechanism enables miss-detected joints to recover meaningful representations by leveraging information from other observed joints. 
Next, for temporal modeling, $H_k$ is reshaped into $\mathbb{R}^{N_1 \times (J \times C_a)}$, forming $N_1$ tokens, each aggregating information across all joints at a given frequency. These tokens are processed by a Frequency Transformer (F-Transformer), which applies self-attention along the temporal dimension to ensure the generated motion sequence is temporally smooth and realistic.

To inject the conditional information, we adopt the Feature-wise Linear Modulation (FiLM) strategy. For the S-Transformer, we maintain joint-wise conditioning by directly inputting $C \in \mathbb{R}^{J \times 384}$, allowing each joint to receive individualized control. For the F-Transformer, which processes joint-aggregated tokens, we apply mean-pooling over the joint dimension to obtain a global condition $C' \in \mathbb{R}^{1 \times 384}$ before applying FiLM.


\subsection{Overall Learning Objective}
\label{overall training}

The Dual-Domain Historical Motion Estimation and Global Skeleton-Cooperative Future Prediction are trained in two separate stages. In the first stage, we train the FDM module to capture the dominant motion trends from noisy radar input. The FDM is supervised using an $L_2$ loss with the GT frequency-domain historical motion as the training target:
\begin{equation}
    \mathcal{L}_{1}=||\tilde{X}^{1:N_2}-\mathcal{F}_{iDCT}^{2}(x^{1:H})||^2.
\end{equation}
Subsequently, based on the pretrained TPR and FDM, we train the GST-based diffusion model in the second stage. The model is optimized using the $\varepsilon$-prediction objective from denoising diffusion probabilistic models (DDPM)~\cite{ho2020denoising}, which minimizes the discrepancy between the predicted and true noise added at each diffusion timestep.
\begin{equation}
    \mathcal{L}_{2}=||\hat{\varepsilon}_{\theta}(X_k, k, C) - \varepsilon_k||^2.
\end{equation}



% As feature extraction from global radar PCs is computation-consuming, we divide the training process into two phases. Phase one facilitates the extraction of the global joint features $F^j$ and coarse estimation of human poses $\tilde{H}$. The GRC, PC encoder (from an off-the-shelf mmWave HPE network), and an MLP-based pose decoder are trained together. The learning objective of the phase one is minimizing the $\mathcal{L}_2$ pose regression loss $\mathcal{L}_{\text{joint}}$:
% \begin{equation}
%     \mathcal{L}_{\text{joint}}={E}_{i \sim[1,17]}|| h^i-\tilde{h}^i \|_2^2.
% \label{loss1}
% \end{equation} 
% In phase two, the remaining three conditional modules and the diffusion model are trained together, with the phase one parameters frozen. The extracted $F^j$ and $\tilde{H}$ serve as the input of structural-motion consistency modules, and $\tilde{H}$ initialize $\hat{H}_K$ for the reverse diffusion process. The learning objective is minimizing $\mathcal{L}_{\text {diff}}$, which is the diffusion learning objective following DDPM~\cite{ho2020denoising}. To ensure accurate limb-length estimation, an $\mathcal{L}_1$ limb regression loss is further designed and integrated:
% \begin{align}
% \begin{split}
%     \mathcal{L}_{\text {diff}}=\mathbb{E}_{k \sim[1, T]} \mathbb{E}_{\varepsilon_k \sim \mathcal{N}(0, I)}|| \varepsilon_k - \hat{\varepsilon}_\theta(H_k, k, C)\|^2_2 \\ + \lambda * \mathbb{E}_{i \sim[1, 16]}|l^i-\hat{l}^i|_1,
% \end{split}
% \label{loss2}
% \end{align}
% where $\lambda$ is a weighting parameter and each $l^i$ is the ground truth limb-length calculated from ground truth pose $H$.



% The Discrete Cosine Transform (DCT) is a widely-used signal processing technique that transforms a sequence of real-valued temporal signals into the frequency domain. For human motion sequences, which are typically smooth and temporally correlated, DCT offers an efficient and compact representation by concentrating the majority of signal energy into a small number of low-frequency components. This property makes DCT particularly effective for motion prediction tasks, where modeling dominant trends while suppressing noise is essential.

% The \textit{Discrete Cosine Transform (DCT)} is a widely-used signal processing technique that transforms a sequence of real-valued temporal signals into the frequency domain. For human motion sequences, which are typically smooth and temporally correlated, DCT offers an efficient representation. It concentrates the majority of signal energy (i.e., overall motion trends) into a small number of low-frequency components and separates motion jitter and noise into high-frequency components.

% This frequency-domain motion representation $\mathbf{X}^{1:N}$ enables efficient and compact modeling of temporally smooth motion, particularly suitable for noisy mmWave modality. 

% In our task, we leverage two different DCT transformation matrices. For historical dominant motion learning, we select $D_1 \in \mathbb{R}^{N_1 \times H}$ for DCT $\mathcal{F}^1_{DCT}$ and iDCT $\mathcal{F}^1_{iDCT}$, designed for transforming $H$-frame historical pose sequences. For future motion prediction with the diffusion model, we select $D_2 \in \mathbb{R}^{N_2 \times (H+F)}$ for DCT $\mathcal{F}^2_{DCT}$ and iDCT $\mathcal{F}^2_{iDCT}$, designed for transforming entire $(H+F)$-frame pose sequences.


